Optimistic MLE -- A Generic Model-based Algorithm for Partially Observable Sequential Decision Making

This paper introduces a simple efficient learning algorithms for general sequential decision making. The algorithm combines Optimism for exploration with Maximum Likelihood Estimation for model estimation, which is thus named OMLE. We prove that OMLE learns the near-optimal policies of an enormously rich class of sequential decision making problems in a polynomial number of samples. This rich class includes not only a majority of known tractable model-based Reinforcement Learning (RL) problems (such as tabular MDPs, factored MDPs, low witness rank problems, tabular weakly-revealing/observable POMDPs and multi-step decodable POMDPs), but also many new challenging RL problems especially in the partially observable setting that were not previously known to be tractable. Notably, the new problems addressed by this paper include (1) observable POMDPs with continuous observation and function approximation, where we achieve the first sample complexity that is completely independent of the size of observation space; (2) well-conditioned low-rank sequential decision making problems (also known as Predictive State Representations (PSRs)), which include and generalize all known tractable POMDP examples under a more intrinsic representation; (3) general sequential decision making problems under SAIL condition, which unifies our existing understandings of model-based RL in both fully observable and partially observable settings. SAIL condition is identified by this paper, which can be viewed as a natural generalization of Bellman/witness rank to address partial observability. This paper also presents a reward-free variant of OMLE algorithm, which learns approximate dynamic models that enable the computation of near-optimal policies for all reward functions simultaneously.

==> outline.tex <==
%! TEX root = main.tex


\section{Outline}
\begin{enumerate}
    \item Intro
    \item Preliminary (interactive decision process, model-based function approximation)
    \item OMLE, generalized Eluder condition, sample complexity bound (put all regret results in appendix).
    \item Weakly revealing PSRs
    \begin{itemize}
        \item Finite observation
        \item Infinite observation
        \item Examples
    \end{itemize}
    \item General PSRs
    \item Low witness rank
    \item Conclusion
    % \begin{itemize}
    %     \item Warm-up weakly-revealing condition for POMDP is not invariant subject to (duplicate state or add dummy state etc)
    %     \item does weakly-revealing POMDP works for (duplicate + minor changes to the state); maybe we can use this as an example.
    % \end{itemize}
    % \item Main results
    % \item Example
    % \begin{itemize}
    %     \item weakly-revealing POMDP
    %     \item m-step decodable POMDP
    %     \item weakly-revealing PSR
    %     \item *weakly-revealing tabular POMDP + Gaussian noisy observation
    %     \item artificial function approximation example?
    % \end{itemize}
\end{enumerate}



% \begin{enumerate}
%     \item Intro
%     \item Preliminary (overcomplete PSR, property)
%     \item Weakly revealing condition
%     \begin{itemize}
%         \item Warm-up weakly-revealing condition for POMDP is not invariant subject to (duplicate state or add dummy state etc)
%         \item does weakly-revealing POMDP works for (duplicate + minor changes to the state); maybe we can use this as an example.
%     \end{itemize}
%     \item Main results
%     \item Example
%     \begin{itemize}
%         \item weakly-revealing POMDP
%         \item m-step decodable POMDP
%         \item weakly-revealing PSR
%         \item *weakly-revealing tabular POMDP + Gaussian noisy observation
%         \item artificial function approximation example?
%     \end{itemize}
% \end{enumerate}

% \chijin{try the assumption if arbitrary action sequence will give weakly-revealing condition in the multi-step setting.}

% \qinghua{check whether generic pomdp fits into witness rank}

% \section{Outline}

% Tabular PSR, PSR with function approximation.
% \begin{enumerate}
%     \item [use citation] relation of POMDPs, OOMs \& PSRs.
%     \item properties of (overparameterized) PSRs
%     \begin{itemize}
%         \item [...] self-consistency
%         \item [?] covering number of tabular PSRs.
%     \end{itemize}
%     \item weakly-revealing assumptions.
%     \item learning in polynomial samples.
% \end{enumerate}

% \noindent Generic OMLE.
% \begin{enumerate}
%     \item generic l2 * log|M|
%     \item fully observable
%     \begin{itemize}
%         \item !witness rank (whether our result is sharper)
%         \item factored MDPs
%         \item [only write if can be done very quickly] linear mixture model
%         \item tabular MDP
%         \item sparse contextual bandit
%     \end{itemize}
%     \item partially observable
%     \begin{itemize}
%         \item !!!generic tabular POMDPs (no assumption)
%         \item weakly-revealing PSR
%         \item weakly revealing tabular POMDPs
%         \item linear transition + linear emission
%         \item ?observable LQR
%     \end{itemize}
% \end{enumerate}

% TODO:
% 1. better normalization condition compatible with POMDP?
% 2. partially observable + witness rank.
% 3. Sharp rate?



\section{Generalized Eluder Dimension}

\begin{definition}\label{defn:model-eluder}
    Given a model class $\mathfrak{M}$ and a policy class $\Pi$, we define the $k$-Eluder dimension of $(\cM,\Pi)$ to be the minimum number $d\in\R$ so that for any $\cM,\cM^1,\ldots,\cM^k\in\mathfrak{M}$, $\pi^1,\ldots,\pi^k\in\Pi$ and $\beta\in\R$, if 
    $$
    \sum_{s=1}^{t-1} \TV^2(\P_{\cM^t}^{\pi^t}, \P_{\cM}^{\pi^t}) \le  \beta \text{ for all } t\in[k],
    $$
    then $\sum_{t=1}^{k} \TV( \P_{\cM^t}^{\pi^t} , \P_{\cM}^{\pi^t}) \le  \sqrt{dk\max\{\beta,1\}}$.
\end{definition}
Here $\P_{\cM}^{\pi}$ denotes the distribution over trajectories generated by executing policy $\pi$ in model $\cM$. We can interpret Definition \ref{defn:model-eluder} as a model-based version of eluder dimension, by viewing models as funcions and policies as points.  

\section{Examples}

\paragraph{Weakly-revealing POMDPs}
\begin{itemize}
    \item Tabular: ${\color{red}\checkmark}$
    \item Block MDPs with no dependence on $\alpha$, simply $\poly(S,A,H,\log|\mathfrak{M}|)$. \yes  \\
    This inspires us to replace the weakly revealing condition by $\|\O^\dagger\|_1 \le 1/\tilde{\alpha}$. Denote $\sigma_S(\O)=\alpha$. We can verify that $\alpha/\sqrt{S} \le \tilde{\alpha} \le \alpha \times \sqrt{O}$. In particular, for block MDPs, $\tilde{\alpha}\equiv1$ but $\alpha$ can be $\Theta(1/\sqrt{O})$. So $\tilde{\alpha}$ seems to be a more intrinsic quantity. And our current proofs work perfectly (are even simplified) with $\tilde{\alpha}$.
     
    \item Function approximation: 
    \begin{itemize}
        \item model-based: suppose the learner is given a family of $\alpha$-weakly revealing POMDPs $\cM$, we want sample complexity $\poly(S,A^m,H,1/\alpha,\log|\cM|)$  \yes
        \item operator-based: given a family of operators $\cB$ that satisfy certain $\gamma$-normalization conditions,  we want sample complexity $\poly(A^m,H,\log|\cB|)$  \notsure \qinghua{It seems to work but we need to discuss whether those properties are too ad hoc.}
    \end{itemize}
\end{itemize}


\paragraph{Witness rank}  \yes

\paragraph{Linear quadractic regulators} 
\begin{itemize}
    \item The covariance matrix of noise is \emph{known} \yes
    \item The covariance matrix of noise is \emph{unknown} \notsure
    \begin{itemize}
        \item Partially observable LQRs can be reduced to LQRs with unknown covariance of noise.
    \end{itemize}
\end{itemize}

\paragraph{Sparse linear bandits} 
\omle~achieves regret $\tilde{\cO}(\sqrt{sdk})$ where $s$ is the sparsity parameter. \yes

\begin{remark}
    When the signal-to-noise ratio is less or equal to $1/d_{E}$, is optimisim the best thing you can do?
\end{remark}

\paragraph{Linear mixture MDPs} \yes \qinghua{Double check if we can get rid of $\log|\cS|$}

\begin{remark}
    By \yes, we mean the \omle algorithm will work for that problem, which is not equivalent to the problem having low model-based eluder dimension.
\end{remark}

\paragraph{Polynomial transitions} Special cases of LQRs.

\begin{remark}
    Open question: \csaba{What if we do not know the size of the minimal POMDP realization?}
\end{remark}

